Runtime Enforcement for Component-Based Systems

Runtime enforcement is an increasingly popular and effective dynamic validation technique aiming to ensure the correct runtime behavior (w.r.t. a formal specification) of systems using a so-called enforcement monitor. In this paper we introduce runtime enforcement of specifications on component-based systems (CBS) modeled in the BIP (Behavior, Interaction and Priority) framework. BIP is a powerful and expressive component-based framework for formal construction of heterogeneous systems. However, because of BIP expressiveness, it remains difficult to enforce at design-time complex behavioral properties. First we propose a theoretical runtime enforcement framework for CBS where we delineate a hierarchy of sets of enforceable properties (i.e., properties that can be enforced) according to the number of observational steps a system is allowed to deviate from the property (i.e., the notion of k-step enforceability). To ensure the observational equivalence between the correct executions of the initial system and the monitored system, we show that i) only stutter-invariant properties should be enforced on CBS with our monitors, ii) safety properties are 1-step enforceable. Given an abstract enforcement monitor (as a finite-state machine) for some 1-step enforceable specification, we formally instrument (at relevant locations) a given BIP system to integrate the monitor. At runtime, the monitor observes and automatically avoids any error in the behavior of the system w.r.t. the specification. Our approach is fully implemented in an available tool that we used to i) avoid deadlock occurrences on a dining philosophers benchmark, and ii) ensure the correct placement of robots on a map.

==> example/Makefile <==
.PHONY: all clean code2bip demiclean listings figures

all: figures listings code2bip

figures:
	$(MAKE) -C figures all

listings:
	$(MAKE) -C listings all

code2bip: listings/dp-philosopher.pdf \
	listings/dp-philosopher-re.pdf \
	listings/dp-fork.pdf \
	listings/dp-fork-re.pdf \
	listings/dp-counter.pdf \
	listings/dp-counter-re.pdf \
	listings/dp-full.pdf \
	listings/dp-full-re.pdf \
	listings/dp-monitor-re.pdf

listings/%.pdf: bip/%.bip
	zsh --interactive -c "bipcolor $< && exit"
	mv $<.pdf $@

demiclean:
	$(MAKE) -C figures demiclean
	$(MAKE) -C listings demiclean
	rm -rf *.aux *.log

clean:
	$(MAKE) -C figures clean
	$(MAKE) -C listings clean
	rm -rf *.pdf *.aux *.log


==> example/figures/Makefile <==
all: \
	dp-trace.pdf \
	dp-trace-re.pdf \
	dp-monitor.pdf \
	dp-monitor-re.pdf \
	dp-counter.pdf \
	dp-counter-re.pdf \
	dp-fork.pdf \
	dp-fork-re.pdf \
	dp-philosopher.pdf \
	dp-philosopher-re.pdf \
	dp-full.pdf \
	dp-full-re.pdf

%.pdf: %.tex
	xelatex $<

demiclean:
	rm -rf *.log *.aux

clean:
	rm -rf *.pdf *.aux *.log


==> example/figures/bipre.tex <==

\newcommand{\portrecover}{$p^r$}
\newcommand{\portmonitor}{$p^m$}
\newcommand{\portcontinue}{$p^c$}
\newcommand{\portname}[1]{$\mathrm{#1}$}

\tikzstyle{monitor}=[->,draw=orange,fill=orange]
\tikzstyle{recover}=[->,draw=red,fill=red]
\tikzstyle{continue}=[->,draw=green!50!black,fill=green!50!black]

\tikzstyle{component}=[auto,node distance=1.0cm,thick,
  align=center,inner sep=0cm,minimum size=0pt,
  ->,>=stealth',shorten >=1pt,
]{}
\tikzstyle{export}=[state,fill=black,minimum size=1.5mm,inner sep=0mm]{}
\tikzstyle{bip}=[auto,node distance=1cm,line width=2pt,>=to,thick,align=center]{}

\newcommand{\component}[3]{
  \node[rectangle,draw] (#1) [#2] {
    \\ \\ \\
    \begin{tikzpicture}[component]
%      \tikzstyle{state}=[state,fill=white!89!black,draw=white!50!black]
      \tikzset{
      place/.style={state,fill=white!89!black,draw=white!50!black,minimum size=0.6cm,inner sep=0cm},
      prime/.style={place,fill=white!95!black,draw=white!70!black}
    }
      #3
    \end{tikzpicture}
  }
}




==> example/listings/Makefile <==
.PHONY: all clean demiclean

all: \
	dp-invariant.pdf \
  dp-meg.pdf \
	dp-monitor-xml.pdf

%.pdf: %.tex
	xelatex -shell-escape $<

demiclean:
	rm -rf *.aux *.log

clean:
	rm -rf *.pdf *.aux *.log




==> proofs.tex <==
\section{Proofs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

In the following proofs, we will consider several mathematical objects in order to prove the correctness of our framework:
\begin{itemize}
 \item a runtime oracle ${\cal O} = (\Theta^{\cal O},$ $\tinit{\cal O}, \Sigma,\trans{}{\cal O},$ $\bfour,\mathit{ver}^{\cal O})$;
\item a BIP enforcement monitor ${\cal E}=(P,L,T,X,$ $\{g_\tau\}_{\tau \in T},$ $\{f_{ \tau}\}_{\tau \in T})$ generated from ${\cal O}$;
\item a composite component $B=\pi(\Gamma(\{B_i\}_{i\in [1,n]}))$ along with its behavior $C=(Q,A,\goesto)$;
\item  the instrumented composite component $B^{rec}=\pi^{\it rec}(\Gamma^{\it rec}(B_1^{\it rec},\ldots,B_n^{\it rec}, {\cal E}))$ by following the procedure described in Definition~\ref{def:connectionsspin}.
The behavior of the instrumented composite component is given by the LTS $C^{rec}=(Q^{rec},A^{rec},\goesto^{rec})$.
%\item  the instrumented composite component $\pi^{\it rec}(\Gamma^{\it rec}(B_1^{\it rec},\ldots,B_n^{\it rec}, {\cal E}, {\cal D}))$ by following the procedure described in Definition~\ref{def:connections}.
\end{itemize}
%
We present the notion of \emph{run} of a composite component.
%
\begin{definition}[Run of a composite component]
\label{def:runcomposite}
A run of length $m$ of a system $(B,\mathit{Init})$ whose runtime semantics is $\pi(C)=(Q,A,\goesto_\pi)$ is the sequence of alternating states and interactions $q^0\cdot a_0\cdot q^1\cdot a_1\cdots a_{m-1}\cdot q^m$ such that: $q^0$ = $\mathit{Init}$, and, $\forall i\in [0,m-1]: q^i\in Q \wedge \exists a_i\in A: q^i \goesto[a_i]_\pi q^{i+1}$.
\end{definition}
%
The set of all runs of $C$ is noted $\Runs(C)$
%

\iffalse
We define the predicates $\sndmon$, $\conmon$, and $\recmon$ such that for a state $q\in Q^{rec}$ and a run $r$, 
\begin{itemize}
\item
$\sndmon(q,r) = \true$ if $\exists n,i\in\mathbb{N}: r = q_0\cdot a_0 \cdots q_i \cdot a_i \cdot q_{i+1}\cdots q_n \wedge q=q_i \wedge {\cal E}.p^m \in a_i$.
\item
$\conmon(q,r) = \true$ if $\exists n,i\in\mathbb{N}: r = q_0\cdot a_0 \cdots q_i \cdot a_i \cdot q_{i+1}\cdots q_n \wedge q=q_i \wedge {\cal E}.p^c \in a_i$,
\item
$\recmon(q,r) = \true$ if $\exists n,i\in\mathbb{N}: r = q_0\cdot a_0 \cdots q_i \cdot a_i \cdot q_{i+1}\cdots q_n \wedge q=q_i \wedge {\cal E}.p^r \in a_i$.
\end{itemize}
\fi


%
\newcommand{\darrow}{{\downarrow}}
%
\begin{definition}[Projecting the run of the monitored system]
The projection of a run $r$ of the monitored system $C^{rec}$ is defined as follows:
\[
\begin{array}{l}
\epsilon \darrow = \epsilon\\
r\darrow =
\left\{
\begin{array}{ll}
r'\darrow \cdot q & \text{if } r=r' \cdot q \cdot a \cdot q' \cdot a_m \cdot q_m \cdot a_r \cdot q \wedge  {\cal E}.p^m \in a_m \wedge  {\cal E}.p^r \in a_r\\
r'\darrow\cdot q\cdot a'\cdot q'' & \text{if } r=r' \cdot q \cdot a' \cdot q' \cdot a_m \cdot q_c \cdot a_c \cdot q'' \wedge  {\cal E}.p^m \in a_m \wedge  {\cal E}.p^c \in a_c\\
r'\darrow \cdot a \cdot q & \text{ if } r = r' \cdot a \cdot q \wedge \{ {\cal E}.p^m, {\cal E}.p^c, {\cal E}.p^r \} \cap a = \emptyset.
\end{array}
\right.
\end{array}
\]
\end{definition}
%
Note that all cases are covered in the above definition because of how components are instrumented and the priorities given to the interactions with the enforcement monitor.

We present how a \emph{run} of a composite component is monitored.
%
\begin{definition}[Monitoring a run of a system]
The verdict ${{\cal O}}(q^0 \cdot a_0 \cdot q^1\cdots a_{m-1}\cdot q^m)$ stated by ${\cal O}$ for a run $q^0 \cdot a_0 \cdot q^1\cdots a_{m-1}\cdot q^m$ is $\mathit{ver}^{\cal O}(\theta^m)$ where $\forall i\in [0,m-1]: \theta_i \trans{e}{\cal O} \theta_{i+1}$ and $e$ is the unique event\footnote{This event is unique because of determinism (see Definition~\ref{def:readiness}).} in $\theta_i$ such that $q^{i+1} \models e$, $\theta_i\in\Theta^{\cal O}$ and $\theta_0=\tinit{\cal O}$.
\end{definition}
%
Any execution of the monitored system is an execution of the initial system.
%That is the monitor selects in the system, among several executions due to non-determinism.
Moreover, any correct execution of the initial system is an execution of the monitored system.
%
\begin{proposition}
$\forall r\in \Runs(C): {\cal O}(r) \in \{\top_c, \top\} \Rightarrow \exists r'\in\Runs(C^{rec}): r = r'\darrow$.
%$\forall r\in \Runs(C), \exists r'\in\Runs(C^{rec}): {\cal O}(r) \in \{\top_c, \top\}\wedge r = r'{\downarrow} \Rightarrow $.
\end{proposition}
%
\begin{proposition}
$\forall r\in \Runs(C^{rec}), \exists r'\in\Runs(C): r'= r{\downarrow}\cdot Q^{*}$.
\end{proposition}
%

\begin{definition}[Stable state]
A state $q\in Q^{rec}$ is said to be \emph{stable},  if $\nexists q'\in Q^{rec}, a \in A^{rec}: q \goesto[a]^{rec} q' \wedge \{ {\cal E}.p^m, {\cal E}.p^c, {\cal E}.p^r \} \cap a \neq \emptyset$.
\end{definition}

\begin{definition}[Stable run]
A run $r \in\Runs(C^{rec})$ is said to be \emph{stable} if $\exists q: last(r) = q \wedge q$ is stable. We denote by $StableRuns$ the set of all runs that are stable. 
\end{definition}




%
\begin{proposition}
$\forall r\in StableRuns: {\cal O}(r\darrow) \in \{\top_c, \top\}$.
\end{proposition}

\begin{proof}

\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Projection on runs.

- erases the states of the monitor 

1.


let B be the initial system, let B_rec = Transform(B) and B_np be system B where the priority model is ignored,

2.

Any execution of the monitored system deviates from the property by at most one step.

let B_rec = Transform(B), for any run r of B_rec, one cannot find two states q,q’ in r s.t. q -> q’ in the run and both q and q’ do not satisfy the property.
\fi
